Perceive to Hypothesize, Verify to Ground: An Agentic Reasoning Framework for Open-World Geo-Localization

Open-world geo-localization requires models to reason over ambiguous visual cues through multi-step reasoning and external knowledge grounding. While recent large vision-language models exhibit strong multimodal reasoning capabilities, existing approaches still suffer from perceptual hallucination and context drift due to the lack of explicit evidence-grounded verification. In this work, we reformulate geo-localization as a human-like perceive-then-verify reasoning problem and propose GeoPAVE (Geo-localization Perception-and-Verification-Engine), a bi-level agentic framework that contains perception-based hypothesis generation via single-pass rollouts and verification-based evidence grounding for decision actions: support, refute, and refine. To support rigorous evaluation, we further introduce PAVED, a novel dataset derived from real-world user check-in data, equipped with comprehensive reasoning trajectories featuring multi-hop queries, multi-round tool invocations, and structured perception-verification traces. The dataset and code are available at https://github.com/Arandinglv/GeoPAVE.

==> latex/tables/other_dataset_table.tex <==
\begin{table*}[htbp]
\centering
\small 
\renewcommand{\arraystretch}{1.3}  % 增加行高，保持与前表一致
\setlength{\tabcolsep}{3pt}        % 稍微缩减列间距以适应11列的宽度

% 使用 tabularx，第一列左对齐(l)，后面10列使用自动拉伸的居中列 C
% 确保导言区定义了 C 列：\newcolumntype{C}{>{\centering\arraybackslash}X}
\begin{tabularx}{\textwidth}{l CCCCC | CCCCC} 
\toprule
\multirow{2}{*}{\textbf{Model}} & \multicolumn{5}{c|}{\textbf{MapBenchV2 (\%)}} & \multicolumn{5}{c}{\textbf{IM2GPS3K (\%)}} \\
\cmidrule(lr){2-6} \cmidrule(lr){7-11}
& 500m & 2km & 25km & 200km & 750km & 500m & 2km & 25km & 200km & 750km \\
\midrule
GeoCLIP              & 0.88  & 1.59  & 6.01  & 12.39 & 32.29 & 8.94  & 18.35 & 32.17 & 49.45 & 66.53 \\
GeoReasoner          & 0.00  & 1.46  & 11.76 & 21.44 & 37.09 & 2.04  & 10.98 & 25.19 & 36.24 & 52.82 \\
GAEA                 & 0.42  & 5.26  & 25.45 & 34.84 & 56.24 & -     & -     & -     & -     & -     \\
GeoVista             & 0.25  & 4.17  & 22.86 & 27.36 & 33.54 & 3.47  & 13.55 & 28.06 & 35.90 & 44.61 \\
GLOBE                & -     & -     & -     & -     & -     & 2.10  & 8.91  & 35.12 & 50.24 & 64.61 \\
Thinking+amap        & 13.73 & 23.20 & 49.52 & 57.95 & 76.60 & -     & -     & -     & -     & -     \\
Thinking*4+3.0flash  & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     \\
SmileGeo             & -     & -     & -     & -     & -     & -     & -     & 47.77 & -     & -     \\
GraphGeo             & -     & -     & -     & -     & -     & -     & -     & 49.15 & -     & -     \\
GPT-5.5              & 7.68  & 18.48 & 34.63 & 43.68 & 58.70 & \textbf{19.19} & \textbf{35.37} & \textbf{56.52} & \textbf{69.44} & \textbf{81.38} \\
\midrule
\rowcolor{tableblue} % 给Ours这一行上色
GeoPAVE (Ours)        & \textbf{13.81} & \textbf{24.83} & \textbf{63.19} & \textbf{70.42} & \textbf{86.87} & 15.92 & 30.51 & 52.30 & 66.18 & 81.24 \\
\bottomrule
\end{tabularx}
\caption{Comparison of geolocation accuracy on MapBenchV2 and IM2GPS3K under different error thresholds. Best results are in bold.}
\label{tab:other_results}
\end{table*}
